Unveiling Covert Semantics: Joint Source-Channel Coding Under a Covertness Constraint

The fundamental limit of Semantic Communications (joint source-channel coding) is established when the transmission needs to be kept covert from an external warden. We derive information-theoretic achievability and matching converse results and we show that source and channel coding separation holds for this setup. Furthermore, we show through an experimental setup that one can train a deep neural network to achieve covert semantic communication for the classification task. Our numerical experiments confirm our theoretical findings, which indicate that for reliable joint source-channel coding the number of transmitted source symbols can only scale as the square-root of the number of channel uses.

==> contents/achievability_proof.tex <==
\subsection{Achievability Proof}
\label{sec:achievability_proof}
The source-channel separation allows us to analyse both the source and channel coding separately.
Recall that the system under this technical separation is depicted in Figure \ref{fig:source_channel_coding}.
% The error probability analysis follows by the lines of \cite{bash_first}.
% We now focus on the analysis of expected distortion.
\subsubsection{Error probability Analysis}
\label{sec:error_proba_analysis}
The error probability analysis follows by the lines of \cite{bash_first}.
One can show that the error probability $\Pr[M \neq \widehat{M} ]$ vanishes in the limit of large blocklength $n$ if
\begin{IEEEeqnarray}{rCl}
     R < \frac{n}{k} \alpha_n \mathbb{D} \left( \Gamma_{Y \mid X}(\cdot \mid 1) \| \Gamma_{Y \mid X}(\cdot \mid 0) \right), \label{eq:channel_coding_proof_condition_on_rate_used_in_collect}
\end{IEEEeqnarray}
% removed for concistency
% Consider the channel coding scheme described in \ref{sec:channel_coding_scheme}.
% In this subsection, we analyse the probability of decoding error averaged over the random codebook $\mathcal{C}_c$.
% For all messages $M, \widehat{M} \in [|1,2^{kR}|]$, we define the decoding error probability
% \begin{equation}
%     \Pr(\mathcal{E}) \triangleq \mathbb{E}_{\mathcal{C}_c} \left[ \Pr(M \neq \widehat{M}) \right].
% \end{equation}
% By the symmetry of the code construction, we can set $M=1$.
% Consider the events
% \begin{IEEEeqnarray}{rCl}
%     \!\!\!\!\!\!\!\!\!\!\!\mathcal{E}_{c,1} &\triangleq& \{X^n(1) \notin \mathcal{A}_{\eta}^{n} \}, \\
%     \!\!\!\!\!\!\!\!\!\!\!\mathcal{E}_{c,2} &\triangleq& \{ (X^n(m), Y^n) \in \mathcal{A}_{\eta}^{n} \quad \forall m \in [|2,2^{kR}|]\}.
% \end{IEEEeqnarray}
% By the union bound, we have
% \begin{equation}
%     \Pr(\mathcal{E}) \leq \Pr(\mathcal{E}_{c,1}) + \Pr(\mathcal{E}_{c,2}), \label{eq:error_proba_decoding_event}
% \end{equation}
% and standard argument \cite{bloch_first} gives
% \begin{equation}
%     \lim_{k \to \infty} \Pr(\mathcal{E}_{c,1}) = 0, \label{eq:error_proba_decoding_event_1_vanishes}
% \end{equation}
% whenever
% \begin{equation}
%     \label{eq:eta_value}
%     \eta < n \alpha_n \mathbb{D} \left( \Gamma_{Y \mid X}(\cdot \mid 1) \| \Gamma_{Y \mid X}(\cdot \mid 0) \right).
% \end{equation}
% In the following, we analyse the second probability term in the RHS of \eqref{eq:error_proba_decoding_event}.
% \begin{IEEEeqnarray}{rCl}
%     \Pr(\mathcal{E}_{c,2}) &=& \Pr \left(\bigcup_{m=2}^{2^{kR}} (X^n(m), Y^n) \in \mathcal{A}_{\eta}^{n} \right) \\
%     &\overset{(a)}{\leq}& \sum_{m=2}^{2^{kR}} \Pr \left((X^n(m), Y^n) \in \mathcal{A}_{\eta}^{n} \right) \\
%     &\overset{(b)}{\leq}& \sum_{m=2}^{2^{kR}} 2^{-\eta} \cdot \left( 1 - \frac{\omega_n^2}{{n}} \right)^{n} \\
%     &=& 2^{kR} \cdot 2^{-\eta} \cdot 2^{- \omega_n^2} \\
%     &=& 2^{kR -\eta} \cdot 2^{- \omega_n^2}  \label{eq:channel_coding_proof_condition_on_rate_1}
% \end{IEEEeqnarray}
% Here (a) follows by the union bound and (b) by the definition of the set $\mathcal{A}_{\eta}^{n}$ in \eqref{eq:set_a_eta_n_def_achievability}.
% Notice that since $\lim_{n \to \infty} \omega_n^2 = 0$, we have $\Pr(\mathcal{E}_{c,2})$ vanishes in the limit of large blocklength $n$ if
% \begin{equation}
%    k R < \eta. \label{eq:channel_coding_proof_condition_on_rate}
% \end{equation}
% Combining~\eqref{eq:error_proba_decoding_event_1_vanishes} and \eqref{eq:channel_coding_proof_condition_on_rate_1} allows us to conclude that
% \begin{equation}
%     \lim_{n \to \infty} \Pr(\mathcal{E}) = 0, \label{eq:error_proba_proof}
% \end{equation}
% if
% \begin{IEEEeqnarray}{rCl}
%      R < \frac{n}{k} \alpha_n \mathbb{D} \left( \Gamma_{Y \mid X}(\cdot \mid 1) \| \Gamma_{Y \mid X}(\cdot \mid 0) \right), \label{eq:channel_coding_proof_condition_on_rate_used_in_collect}
% \end{IEEEeqnarray}
% which completes the error probability analysis.
\subsubsection{Analysis of Expected Distortion}
\label{sec:expected_distortion_analysis}
Consider the source coding scheme described in \ref{sec:coding_scheme}.
In the following, we bound the distortion averaged over the random choice of the source coding codebook $\mathcal{C}_s$.

Let $0 < \epsilon' < \epsilon$ and let $M, \widehat{M} \in [|1,2^{kR}|]$ be the index chosen by the source encoder and the channel decoder respectively, see the Figures \ref{fig:source_encoding} and \ref{fig:channel_decoding}.
% \begin{figure}
%     \centering
%     \includegraphics{figures/source_encoder.pdf}
%     \caption{The source encoder}
%     \label{fig:source_encoding}
% \end{figure}
\begin{figure}
    \centering
    \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{figures/source_encoder.pdf}
        \caption{The source encoder.}
        \label{fig:source_encoding}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=0.65\linewidth]{figures/channel_decoder.pdf}
        \caption{The channel decoder}
        % \caption{The channel decoder. It observes the channel output $Y^n$ and produce the guess $\widehat{M}$.}
        \label{fig:channel_decoding}
    \end{minipage}
    % \caption{Overall caption for both figures}
    % \label{fig:both}
\end{figure}

Further define the encoding error event
% In the following, we bound the distortion averaged over the random choice of the codebook $\mathcal{C}_s$, for that we define the encoding error event
\begin{equation}
    \mathcal{E}_s \triangleq \{(U^k, \widehat{U}^k(\widehat{M})) \notin \mathcal{T}_{\epsilon}^{(k)} \},
\end{equation}
as well as the events
\begin{IEEEeqnarray}{rCl}
    \!\!\!\!\!\!\!\mathcal{E}_{s,1} &\triangleq& \{U^k \notin \mathcal{T}_{\epsilon'}^{(k)} \}, \\
    \!\!\!\!\!\!\!\mathcal{E}_{s,2} &\triangleq& \{U^k \in \mathcal{T}_{\epsilon'}^{(k)}, (U^k, \widehat{U}^k(\widehat{M}')) \notin \mathcal{T}_{\epsilon}^{(k)}, \nonumber \\
    && \hspace{1.7cm} M = \widehat{M}' , \quad \forall \widehat{M}' \in [|1,2^{kR}|] \}, \\
    \!\!\!\!\!\!\!\mathcal{E}_{s,3} &\triangleq& \{U^k \in \mathcal{T}_{\epsilon'}^{(k)}, (U^k, \widehat{U}^k(\widehat{M}')) \notin \mathcal{T}_{\epsilon}^{(k)}, \nonumber \\
    && \hspace{1.7cm} M \neq \widehat{M}' , \quad \forall \widehat{M}' \in [|1,2^{kR}|] \},
\end{IEEEeqnarray}
and notice that by the union bound, we have
\begin{IEEEeqnarray}{rCl}
    \!\!\!\!\!\!\!\!\Pr(\mathcal{E}_s) &\leq& \Pr(\mathcal{E}_{s,1}) +  \Pr(\mathcal{E}_{s,2}) + \Pr(\mathcal{E}_{s,3})  \label{eq:error_proba_encoding_event}
\end{IEEEeqnarray}
% \begin{IEEEeqnarray}{rCl}
%     \!\!\!\!\!\!\!\!\Pr(\mathcal{E}_s) &\leq& \Pr(\mathcal{E}_{s,1}) + \sum_{\widehat{m}'=1}^{2^{kR}} \Pr[M = \widehat{m}' ] \cdot \Pr(\mathcal{E}_{s,2}) \nonumber \\
%     && \hspace{0.2cm} + \Pr[M \neq \widehat{M} ] \cdot \Pr(\mathcal{E}_{s,3}) \\ 
%     &\leq& \Pr(\mathcal{E}_{s,1}) + \Pr(\mathcal{E}_{s,2}) + \Pr[M \neq \widehat{M} ] \cdot \Pr(\mathcal{E}_{s,3}) \label{eq:error_proba_encoding_event}
% \end{IEEEeqnarray}
By standard argument,
\begin{equation}
    \lim_{k \to \infty} \Pr(\mathcal{E}_{s,1}) = 0. \label{eq:error_proba_encoding_event_1_vanishes}
\end{equation}
% Moreover, if $R$ satisfies \eqref{eq:channel_coding_proof_condition_on_rate_used_in_collect} then the second term in the right-hand-side (RHS) of \eqref{eq:error_proba_encoding_event} vanishes exponentially fast as 
% $\Pr(\mathcal{E}_{s,1})$ vanishes for sufficiently large $k$.
Regarding the second term in the right-hand-side (RHS) of~\eqref{eq:error_proba_encoding_event}, we have
\begin{IEEEeqnarray}{rCl}
    \lefteqn{\Pr(\mathcal{E}_{s,2})} \nonumber \\
    &=& \Pr \Big(U^k \in \mathcal{T}_{\epsilon'}^{(k)}, (U^k, \widehat{U}^k(\widehat{M}')) \notin \mathcal{T}_{\epsilon}^{(k)},  \nonumber \\
    && \hspace{2.5cm} M = \widehat{M}' , \quad \forall \widehat{M}' \in [|1,2^{kR}|] \Big) \\
    &\overset{(a)}{=}& \Pr[\widehat{M}' = 1] \sum_{u^k \in \mathcal{T}_{\epsilon}^{(k)}} P_U^{\otimes k}(u^k)  \Pr \Big((u^k, \widehat{U}^k(1)) \notin \mathcal{T}_{\epsilon}^{(k)} \nonumber \\
    && \hspace{3cm} \Big| U^k = u^k, \widehat{M}' = 1\Big)^{2^{kR}}\label{eq:step_for_joint_typ_lemme_source_coding}
\end{IEEEeqnarray}
where \eqref{eq:step_for_joint_typ_lemme_source_coding} holds by the symmetry of the code construction.
By the joint typicality Lemma, we have
\begin{IEEEeqnarray}{rCl}
    \lefteqn{\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\Pr \left((u^k, \widehat{U}^k(1)) \notin \mathcal{T}_{\epsilon}^{(k)} \mid U^k = u^k, \widehat{M}' = 1\right)} \nonumber \\
    &\leq& 1 - 2^{-k \left( \mathbb{I}(U;\widehat{U}) + \delta(\epsilon) \right )}.  \label{eq:joint_typ_lemme_source_coding}
\end{IEEEeqnarray}
Plugging \eqref{eq:joint_typ_lemme_source_coding} in \eqref{eq:step_for_joint_typ_lemme_source_coding} yields
\begin{IEEEeqnarray}{rCl}
   \!\!\!\!\!\!\!\!\!\!\! \Pr(\mathcal{E}_{s,2}) &\leq& \sum_{u^k \in \mathcal{T}_{\epsilon}^{(k)}} P_U^{\otimes k}(u^k) \left( 1 - 2^{-k \left( \mathbb{I}(U;\widehat{U}) + \delta(\epsilon) \right )} \right)^{2^{kR}} \\
    & \overset{(a)}{\leq}& \exp \left(-2^{kR} \cdot 2^{-k \left( \mathbb{I}(U;\widehat{U}) + \delta(\epsilon) \right )} \right) \\
    &=& \exp \left(-2^{k \left( R - \mathbb{I}(U;\widehat{U}) - \delta(\epsilon) \right )} \right). \label{eq:error_proba_encoding_event_2_vanishes}
\end{IEEEeqnarray}
where (a) holds by the identity $(1-x)^n \leq \exp(-nx)$ for small values of $x$ around $0$. Therefore $\Pr(\mathcal{E}_{s,2})$ is vanishing if
\begin{equation}
    R > \mathbb{I}(U;\widehat{U}) + \delta(\epsilon). \label{eq:source_coding_proof_condition_on_rate}
\end{equation}
Similarly, one can show that 
\begin{equation}
    \lim_{k \to \infty} \Pr(\mathcal{E}_{s,3}) = 0. \label{eq:error_proba_encoding_event_3_vanishes}
\end{equation}
if \eqref{eq:channel_coding_proof_condition_on_rate_used_in_collect} and \eqref{eq:source_coding_proof_condition_on_rate} are met.
Therefore, we conclude that the encoding error event $\mathcal{E}_s$ has a vanishing probability for $k \to \infty$ if \eqref{eq:channel_coding_proof_condition_on_rate_used_in_collect} and \eqref{eq:source_coding_proof_condition_on_rate} are met.

Further define
\begin{IEEEeqnarray}{rCl}
    \mathcal{D}_1 & \triangleq & \Pr(\mathcal{E}_s) \mathbb{E} \left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \mid \mathcal{E}_s, M = \widehat{M}  \right] \nonumber \\ 
     && \hspace{0.05cm} + (1 - \Pr(\mathcal{E}_s)) \mathbb{E}\left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \mid \mathcal{E}_s^c, M = \widehat{M}  \right], \nonumber \\ \label{eq:expected_distotion_step_typ_avg_lemma_D_1}
\end{IEEEeqnarray}
and
\begin{IEEEeqnarray}{rCl}
    \mathcal{D}_2& \triangleq & \Pr(\mathcal{E}_s) \mathbb{E} \left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \mid \mathcal{E}_s, M \neq \widehat{M}  \right] \nonumber \\ 
     && \hspace{0.05cm} + (1 - \Pr(\mathcal{E}_s)) \mathbb{E} \left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \mid \mathcal{E}_s^c, M \neq \widehat{M}  \right], \nonumber \\ \label{eq:expected_distotion_step_typ_avg_lemma_D_2}
\end{IEEEeqnarray}
where expectations are over the codebook $\mathcal{C}_s$ and the source sequences $U^k$ and consider now the average over the codebook of the distortion.
Notice that by the total law of probabilities we have
\begin{IEEEeqnarray}{rCl}
   \lefteqn{\mathbb{E}_{\mathcal{C}_s, U^k} \left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \right]} \nonumber \\
   &=& \Pr[M = \widehat{M} ] \cdot \mathcal{D}_1 + \Pr[M \neq \widehat{M} ] \cdot \mathcal{D}_2 \\
   &\leq& \mathcal{D}_1 + \Pr[M \neq \widehat{M} ] \cdot \mathcal{D}_2 
\end{IEEEeqnarray}
% \begin{IEEEeqnarray}{rCl}
%     \lefteqn{\mathbb{E}_{\mathcal{C}_s, U^k} \left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \right]} \nonumber \\
%      &=& \Pr(\mathcal{E}_s) \mathbb{E}_{\mathcal{C}_s, U^k} \left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \mid \mathcal{E}_s \right] \nonumber \\ 
%      && \hspace{0.1cm} + (1 - \Pr(\mathcal{E}_s)) \mathbb{E}_{\mathcal{C}_s, U^k} \left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \mid \mathcal{E}_s^c \right] \label{eq:expected_distotion_step_typ_avg_lemma}%\\
%      % &\leq& \Pr(\mathcal{E}) d_{max} + (1 - \Pr(\mathcal{E})) \mathbb{E}_{\mathcal{C}_s, U^k} \left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \mid \mathcal{E}^c \right]. \nonumber \\
% \end{IEEEeqnarray}
Using the typical average Lemma, we upper-bound the second term on the RHS of~\eqref{eq:expected_distotion_step_typ_avg_lemma_D_1}. Therefore, we have:
\begin{IEEEeqnarray}{rCl}
    \lefteqn{\!\!\!\!\!\!\!\!\!\!\mathbb{E}_{\mathcal{C}_s, U^k} \left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \mid \mathcal{E}_s^c, M = \widehat{M} \right]} \nonumber \\
    &=& \frac{1}{k} \sum_{i=1}^k \mathbb{E}_{\mathcal{C}, U_i}[d(U_i,\widehat{U}_i(\widehat{M})) \mid \mathcal{E}_s^c, M = \widehat{M}] \\
    &\leq& (1+\epsilon) \mathbb{E}_{\mathcal{C}, U}[d(U,\widehat{U}(\widehat{M})) \mid \mathcal{E}_s^c, M = \widehat{M}] \\
    &\overset{(a)}{\leq}& (1+\epsilon) \cdot \frac{D}{1+\epsilon} \\
    &=& D. \label{eq:avg_distortion_proof_epsilon_conjugate}
\end{IEEEeqnarray}
Here (a) hold as our source coding scheme is assumed to achieve a distortion $\frac{D}{1+\epsilon}$.

Since the distortion measure $d(\cdot, \cdot)$ is assumed to be bounded, combining \eqref{eq:error_proba_encoding_event_1_vanishes}, \eqref{eq:error_proba_encoding_event_2_vanishes}, \eqref{eq:avg_distortion_proof_epsilon_conjugate} yields
\begin{equation}
    \limsup_{k \to \infty} \mathbb{E}_{\mathcal{C}_s, U^k} \left[ \frac{1}{k} \sum_{i=1}^k d(U_i,\widehat{U}_i(\widehat{M})) \right] \leq D, \label{eq:avg_distortion_proof}
\end{equation}
% if \eqref{eq:source_coding_proof_condition_on_rate} holds.
if
\begin{IEEEeqnarray}{rCl}
    R &>& \mathbb{I}(U;\widehat{U}) + \delta(\epsilon) \\
    &=& R \left(\frac{D}{1+\epsilon} \right) + \delta(\epsilon), \label{eq:source_coding_proof_condition_on_rate_used_in_collect}
\end{IEEEeqnarray}
and
\begin{IEEEeqnarray}{rCl}
     R < \frac{n}{k} \alpha_n \mathbb{D} \left( \Gamma_{Y \mid X}(\cdot \mid 1) \| \Gamma_{Y \mid X}(\cdot \mid 0) \right),
\end{IEEEeqnarray}
which completes the expected distortion analysis.
\subsection{Collecting the results and asymptotics analysis}
\label{sec:collecting_results}
By putting together \eqref{eq:source_coding_proof_condition_on_rate_used_in_collect} and \eqref{eq:channel_coding_proof_condition_on_rate_used_in_collect} we can conclude that for covert communication to be possible in a joint source-channel coding scheme, it must hold that
\begin{equation}
    \mathbb{I}(U;\widehat{U}) \leq \frac{n}{k} \alpha_n \mathbb{D} \left( \Gamma_{Y \mid X}(\cdot \mid 1) \| \Gamma_{Y \mid X}(\cdot \mid 0) \right). \label{eq:condition_on_mutual_info_U_U_hat_before_asymp}
\end{equation}
Moreover, by~\cite[Lemma 1]{bloch_first}
\begin{IEEEeqnarray}{rCl}
    \lefteqn{\mathbb{D}\left(\widehat{Q}^{n} \; \big\| \; \Gamma^{\otimes n}_{Z|X} ( \cdot | 0^n)\right)} \nonumber \\
    &=& ( 1+ o(1)) \frac{\omega_n^2}{2}\chi_2(\Gamma_{Z \mid X}(\cdot \mid 1) \| \Gamma_{Z \mid X}(\cdot \mid 0)).
\end{IEEEeqnarray}
Therefore, we notice that \eqref{eq:condition_on_mutual_info_U_U_hat_before_asymp} is non vanishing and bounded in the asymptotic regime only if one sets
\begin{equation}
    k = \frac{\sqrt{n \delta_n}}{\gamma}. \qquad \forall \gamma \geq 1
\end{equation}
This yields
\begin{IEEEeqnarray}{rCl}
    % \!\!\!\!\!\!\!\!\!\!\mathbb{I}(U;\widehat{U}) &\leq& \lim_{n\to \infty} \sqrt{\frac{n \gamma}{\delta_n}} \mathbb{I}(X;Y) \\
    \lefteqn{\mathbb{I}(U;\widehat{U})} \nonumber \\
    &\leq& \lim_{n\to \infty} \sqrt{\frac{n}{\delta_n}}  \gamma  \alpha_n \mathbb{D} \left( \Gamma_{Y \mid X}(\cdot \mid 1) \| \Gamma_{Y \mid X}(\cdot \mid 0) \right) \\ \label{eq:asymp_condition_on_mutual_info_U_U_hat}
    &=& \lim_{n\to \infty}  \gamma  \frac{\sqrt{n \alpha_n^2} \mathbb{D} \left( \Gamma_{Y \mid X}(\cdot \mid 1) \| \Gamma_{Y \mid X}(\cdot \mid 0) \right)} {\sqrt{( 1+ o(1)) \frac{\omega_n^2}{2}\chi_2(\Gamma_{Z \mid X}(\cdot \mid 1) \| \Gamma_{Z \mid X}(\cdot \mid 0))}} \\
    &=& \sqrt{2} \gamma  \frac{\mathbb{D} \left( \Gamma_{Y \mid X}(\cdot \mid 1) \| \Gamma_{Y \mid X}(\cdot \mid 0) \right)} {\sqrt{\chi_2(\Gamma_{Z \mid X}(\cdot \mid 1) \| \Gamma_{Z \mid X}(\cdot \mid 0))}}. \label{eq:asymp_condition_on_mutual_info_U_U_hat}
\end{IEEEeqnarray}
% To get the $\beta$ constant, one can consider that communication is happening over a fraction $\beta$ of the blocklength $n$, where the transmitter sends a codeword in the first $\beta n$ while it sends only the 0-symbol in the remaining $(1-\beta) n$ slots, thereby completing our achievability proof.
Finally, recalling again that
\begin{IEEEeqnarray}{rCl}
R(D) & = & \min_{P_{\widehat{U} \mid U}(\widehat{u} \mid u) : \mathbb{E}_{P_UP_{\widehat{U} \mid U}} \left[ d(\widehat{U}, U) \right] \leq D } \mathbb{I}(\widehat{U}, U),
\end{IEEEeqnarray}
then it must hold that
\begin{IEEEeqnarray}{rCl}
    \!\!\!\!\!\!\!\!\!\! R(D) &\leq& \sqrt{2} \gamma \frac{ \mathbb{D} \left( \Gamma_{Y \mid X}(\cdot \mid 1) \| \Gamma_{Y \mid X}(\cdot \mid 0) \right)} {\sqrt{\chi^2(\Gamma_{Z \mid X}(\cdot \mid 1) \| \Gamma_{Z \mid X}(\cdot \mid 0)) }}.
\end{IEEEeqnarray}
which completes the achievability analysis.

==> contents/coding_scheme.tex <==
\subsection{A coding Scheme}% Achieving Theorem \ref{main_theorem}}
\label{sec:coding_scheme}
Choose a good source coding scheme \cite{cover} and a good channel coding scheme for covert communication \cite{bloch_first}.
Our approach relies on the technique of source-channel separation and we shall show in the following that this scheme is indeed optimal.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/source_channel_coding.pdf}
    \caption{The source and channel coding separation.}
    \label{fig:source_channel_coding}
\end{figure}

More specifically, the transmitter initially compresses the source sequence $U^k$ into an index $M$ which is subsequently encoded into a codeword $X^n$ and sent through the DMC.
A channel decoder observe $Y^n$, a noisy version of $X^n$, and it maps it to the guessed index.
The latter is used by the source decoder to produce the guess $\widehat{U}^k$, see Figure \ref{fig:source_channel_coding}.

Notice that according to this scheme, an error occurs if the channel decoder miss-decodes the correct index $M$, i.e. $\widehat{M} \neq M$ or if the source decoder is unable to satisfy \eqref{eq:avg_distortion_def}.


% \subsection{Useful Definitions}
% Prior to presenting our coding scheme, we establish the following definitions.
% Let $\{\omega_{n}\}_{n=1}^\infty$ be a sequence satisfying 
% \begin{subequations}   
%     \label{eq:lim_omega_n_def}
%     \begin{IEEEeqnarray}{rCl}
%         \lim_{n \rightarrow \infty} \omega_{n} &=& 0, \\  
%           \lim_{n \rightarrow \infty}\left( \omega_{n}\sqrt{n} -\log n\right) &=& \infty,
%     \end{IEEEeqnarray}
% \end{subequations}    
% and for a positive constant $\epsilon_t$, define 
% \begin{equation}\label{eq:alphan}
%  \alpha_n \triangleq \frac{\omega_n}{\sqrt{n}} \epsilon_t.
% \end{equation}

%% REMOVED for simplicity of presentation
% \subsection{Source Coding}\label{sec:source_coding_cheme}
% Fix a blocklength $n$ and an $\epsilon > 0$.
% Recall the definition of the rate-distortion function
% \begin{IEEEeqnarray}{rCl}
% R(D) & \triangleq & \min_{P_{\widehat{U} \mid U}(\widehat{u} \mid u) : \mathbb{E}_{P_UP_{\widehat{U} \mid U}} \left[ d(\widehat{U}, U) \right] \leq D } \mathbb{I}(\widehat{U}, U).
% \end{IEEEeqnarray}
% Fix a conditional pmf $P_{\widehat{U} \mid U}$ that attains $R(\frac{D}{1+\epsilon})$ with $D$ being the desired maximum distortion, then compute $P_{\widehat{U}}$ the marginal of the joint pmf $P_{\widehat{U}, U}$, i.e.
% \begin{IEEEeqnarray}{rCl}
% P_{\widehat{U}}(\widehat{u}) = \sum_{u \in \mathcal{U}} P_{U}(u) P_{\widehat{U} \mid U}(\widehat{u},u), \quad \forall \widehat{u} \in \mathcal{\widehat{U}}.
% \end{IEEEeqnarray}
% \noindent\underline{\textit{Codebook generation:}}
% Define
% \begin{equation}
%     R \triangleq \frac{\log_2(\mathsf{U})}{k},
% \end{equation}
% and generate the codebook
% % Generate $2^{kR}$ sequences $\widehat{U}^k(m)$ for all $m \in [|1,2^{kR}|]$ i.i.d. according to the pmf $P_{\widehat{U}}^{\otimes k}(\widehat{u}^k(m))$.
% \begin{equation}
%     \mathcal{C}_s =  \left \{\widehat{u}^{k}(1), \ldots, \widehat{u}^{k}\left(2^{kR}\right) \right \} ,
% \end{equation}
% by drawing the $i$-th entry of codeword $\widehat{u}^k(m)$ according to the pmf $P_{\widehat{U}}(\widehat{u}_i(m))$ independent of all other entries, for all $m \in [|1,2^{kR}|]$.
% The codebook $\mathcal{C}_s$ is revealed to all parties.
% \noindent\underline{\textit{Encoding:}}\\
% We use a joint typicality encoding, i.e. for a given input sequence $u^k$, we look for an index $m$ such that $(u^k, \widehat{u}^k(m)) \in \mathcal{T}^{(k)}_{\epsilon}$.
% If there are multiple indices, we choose the smallest one.
% On the other hand, if there are no such index, we set $m=1$.
% \noindent\underline{\textit{Decoding:}}\\
% Upon receiving the index $m$, the legitimate receiver reconstructs the sequence $\widehat{u}^k = \widehat{u}^k(m)$ by a simple look-up from the codebook $\mathcal{C}_s$.
% \subsection{Channel Coding}\label{sec:channel_coding_scheme}
% Let $\{\omega_{n}\}_{n=1}^\infty$ be a sequence satisfying 
% \begin{subequations}   
%     \label{eq:lim_omega_n_def}
%     \begin{IEEEeqnarray}{rCl}
%         \lim_{n \rightarrow \infty} \omega_{n} &=& 0, \\  
%           \lim_{n \rightarrow \infty}\left( \omega_{n}\sqrt{n} -\log n\right) &=& \infty,
%     \end{IEEEeqnarray}
% \end{subequations}    
% and define 
% \begin{equation}\label{eq:alphan}
%  \alpha_n \triangleq \frac{\omega_n}{\sqrt{n}}.
% \end{equation}
% % Fix a blocklength $n$.
% Fix a large blocklength $n$ and let $\{\omega_n\}_{n \in \mathbb{N}}$ be a sequence satisfying \eqref{eq:lim_omega_n_def} and define $\{\alpha_n\}_{n \in \mathbb{N}}$ as in \eqref{eq:alphan}. 
% Define the pmf $P_{X_{n}}$ over $\mathcal{X}$ as
% \begin{IEEEeqnarray}{rCl}
% P_{X_{n}}(1) &= & \alpha_n.
% \end{IEEEeqnarray}
% Moreover, we define the joint pmf
% \begin{equation}\label{eq:Pn}
% P_{XY}^{(n)}\triangleq P_{X_{n}}\Gamma_{Y \mid X}.
% \end{equation}
% % Let $P_{TY}$ denote the $(T,Y)$-marginal of the pmf $P_{TXY}^{(n)}$ and notice that the following asymptotic quantity exists  because for any $t \in \mathcal{T}$ we have $\alpha_n \to 0$:
% % \begin{equation}
% % P_{TY}^*(t,y)\triangleq \lim_{n\to\infty} P_{TY}^{(n)}(t,y) = P_{T}(t)\Gamma_{Y|X}(y|0).
% % \end{equation}
% \noindent\underline{\textit{Codebook generation:}}
% % Let $R_s$ denote the secret-key rate, i.e.
% % \begin{equation}
% %     R_s \triangleq \frac{\log_2(\mathsf{S})}{k}.
% % \end{equation}
% Generate the codebook
% \begin{equation}
%     \mathcal{C}_c =  \left \{  x^{n}(1), \ldots, x^{n}\left(2^{kR}\right) \right \} ,
% \end{equation}
% by drawing the $i$-th entry of codeword $x^n(m)$ according to the pmf $P_{X_n}(\cdot)$ independent of all other entries, for all $m \in [|1,2^{kR}|]$.
% The codebook $\mathcal{C}_c$ is revealed to all parties.
% \noindent\underline{\textit{Encoding:}}\\
% Under $\mathcal{H}=0$ the transmitter sends the sequence $0^n$ over the channel.
% Under $\mathcal{H}=1$ and for every tuple $(m) \in [|1,2^{kR}|]$, the transmitter looks for the corresponding codeword $x^n(m,s)$ from the codebook $\mathcal{C}_c$ and send it over the channel.\\
% \noindent\underline{\textit{Decoding:}}\\
% The legitimate receiver, who observes $Y^n=y^n$ and knows the true hypothesis $\mathcal{H}$, performs a joint typicality decoding.
% More specifically, under $\mathcal{H}=0$, the legitimate receiver abstains from action, whereas under $\mathcal{H}=1$, it looks for a unique index $m$ satisfying 
% \begin{equation}\label{eq:decoding_user_3}
% (x^{n}(m), y^{n}) \in \mathcal{A}_{\eta}^{n},
% \end{equation}
% where
% \begin{IEEEeqnarray}{rCl}
% \label{eq:set_a_eta_n_def_achievability}
% \mathcal{A}_{\eta}^{n} \triangleq \left \{  (x^{n}, y^{n}) \colon  \log \left( \frac{\Gamma_{Y|X}^{\otimes n}(y^{n} | x^{n}) }{\Gamma_{Y|X}^{\otimes n}(y^{n} |0^n) }  \right) \geq \eta \right \}
% \end{IEEEeqnarray}
% and $\eta$ is a constant that is defined later on. 
% If such a unique index  $m$ exists, the receiver sets $\widehat{M}=m$. Otherwise it declares an error and stops.
% % Under $\mathcal{H}=0$, the legitimate receiver does nothing.

==> contents/proofs_michele_edited.tex <==
%\section{Proof of Theorem~\ref{main_theorem}}
%\label{sec:proofs}

%\input{contents/coding_scheme}
\input{contents/converse_proof}
%\input{contents/achievability_proof}


==> contents/resolvability.tex <==
\begin{appendices}

\section{Channel Resolvability Analysis}


Recall that the warden's output distribution under $\mathcal{H}=1$ for a given codebook $\mathcal{C}$ is:
\begin{IEEEeqnarray}{rCl}
\widehat{Q}^{n}(z^{n}) &\triangleq&  \frac{1}{\mathsf{S}} \sum_{(u^k,s)} P_U^{\otimes k}(u^k) \Gamma^{\otimes n}_{Z|X} (z^n| x^n(u^k, s)),
\end{IEEEeqnarray}
whereas the covertness constraint is given by
\begin{equation}
\delta_{n}\triangleq \mathbb{D}\left(\widehat{Q}^{n} \; \big\| \; \Gamma^{\otimes n}_{Z|X} ( \cdot | 0^n)\right).
\end{equation}
In this section, we show the limit
\begin{equation}
\lim_{n \to \infty} \mathbb{E}_{\mathcal{C}}\left[\mathbb{D}\left( \widehat{Q}^{n} \; \big\| \; \Gamma^{\otimes n}_{Z|X} ( \cdot | 0^n) \right) \right] = 0,
\end{equation}
where expectation is with respect to the random code construction. 
We start by  expanding the  divergence of interest as follows:
\begin{align}
    \label{eqn:resolvability_first_steps}
    \lefteqn{
    \mathbb{D}\left( \widehat{Q}^{n} \Big\| \Gamma^{\otimes n}_{Z|X} ( \cdot | 0^n)\right) } \nonumber \\
    &= \mathbb{D}\left( \widehat{Q}^{n} \Big\| Q_{\alpha_n}^{\otimes n}\right) + \mathbb{D}\left( Q_{\alpha_n}^{\otimes n} \Big\| \Gamma^{\otimes n}_{Z|X} ( \cdot | 0^n)\right) \nonumber \\
    &\hspace{0.2cm}+ \sum_{z^n} \left(\widehat{Q}^{n}(z^n) - Q_{\alpha_n}^{\otimes n}(z^n) \right ) \log \left( \frac{Q_{\alpha_n}^{\otimes n}(z^n)}{\Gamma^{\otimes n}_{Z|X} ( \cdot | 0^n)} \right ).
\end{align}
Defining $\nabla_0$ as the minimum probability in the support of $\Gamma_{Z \mid X}(z|0)$:
\begin{equation}\nabla_0 = \min_{z,x_3 \in \text{supp}(\Gamma_{Z \mid X}(z|0))} \Gamma_{Z \mid X}(z|0),
\end{equation} 
 by Pinsker's inequality\footnote{For any two distributions $P$ and $Q$ on the same alphabet $\mathcal{X}$ we have $\mathbb{V}(P,Q) \leq  \sqrt{\frac{\mathbb{D}(P,Q)}{2}}$.}, we can conclude the following:
\begin{align}
    \label{eq:resolvability_original}
    &\left | \mathbb{D}\left( \widehat{Q}^{n} \Big\| \Gamma^{\otimes n}_{Z|X} ( \cdot | 0^n)\right) -  \mathbb{D}\left( Q_{\alpha_n}^{\otimes n} \Big\| \Gamma^{\otimes n}_{Z|X} ( \cdot | 0^n)\right) \right | \\
    &\leq \mathbb{D}\left( \widehat{Q}^{n} \Big\| Q_{\alpha_n}^{\otimes n}\right) + n \log\left( \frac{1}{\nabla_0} \right)  \sqrt{\frac{1}{2}\mathbb{D}\left( \widehat{Q}^{n} \Big\| Q_{\alpha_n}^{\otimes n}\right)}. \label{eq:abs_diff}
\end{align}
We shall separately analyze the divergences $\mathbb{D}( Q_{\alpha_n}^{\otimes n} \| \Gamma^{\otimes n}_{Z|X} ( \cdot | 0^n))$  and $\mathbb{D}\left( \widehat{Q}^{n} \Big\| Q_{\alpha_n}^{\otimes n}\right)$, or more precisely their expectations over the choices of the codebooks.

\textit{Analysis of the expected divergence $\mathbb{D}\left( \widehat{Q}_{\mathcal{C}, w_3}^n \Big\| Q_{\alpha_n}^{\otimes n}\right)$:}
Consider the average (over the codebooks) expected divergence
\begin{IEEEeqnarray}{rCl}  
 \lefteqn{  \mathop{\mathbb{E}}_{ \{X^{n}(U^k,S)\}}\left[\mathbb{D}\left( \widehat{Q}_{\mathcal{C}}^n \Big\| Q_{\alpha_n}^{\otimes n}\right) \right]}\nonumber\\
&=& \mathbb{E} \left [\sum_{z^n}  \widehat{Q}_{\mathcal{C}}^{n}(z^{n})\log \left( \frac{ \widehat{Q}_{\mathcal{C}}^{n}(z^{n} )}{Q_{\alpha_n}^{\otimes n}(z^n) } \right) \right] \\[1.2ex]
&=& \mathbb{E} \left [\sum_{z^n} \frac{1}{\mathsf{S}} \sum_{(u^k,s)} P_U^{\otimes k}(u^k) \Gamma^{\otimes n}_{Z|X} (z^n| x^n(u^k, s)) \nonumber \\
&&\hspace{0.1cm} \cdot \log \left( \frac{ \sum_{(u^k,s)} P_U^{\otimes k}(u^k) \Gamma^{\otimes n}_{Z|X} (z^n| x^n(u^k, s))}{S Q_{\alpha_n}^{\otimes n}(z^n) } \right) \right] \\[1.2ex]
\end{IEEEeqnarray}








\end{appendices}

==> references_old.tex <==
% book links kl divergence to detection error proba
@book{hypo_test_book,
	doi = {10.1007/0-387-27605-x},
	url = {https://doi.org/10.1007%2F0-387-27605-x},
	year = 2005,
	publisher = {Springer New York},
	title = {Testing Statistical Hypotheses}
}

% AWGN first Bash
@ARTICLE{bash_first,
  author={Bash, Boulat A. and Goeckel, Dennis and Towsley, Don},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Limits of Reliable Communication with Low Probability of Detection on AWGN Channels}, 
  year={2013},
  volume={31},
  number={9},
  pages={1921-1930},
  doi={10.1109/JSAC.2013.130923}}
  
% Point-toPoint
@ARTICLE{bash_p2p,
author={Bash, Boulat A. and Goeckel, Dennis and Towsley, Don and Guha, Saikat},
journal={IEEE Communications Magazine}, 
title={Hiding information in noise: fundamental limits of covert wireless communication}, 
year={2015},
volume={53},
number={12},
pages={26-31},
doi={10.1109/MCOM.2015.7355562}}




@ARTICLE{bloch_first,
author={Bloch, Matthieu R.},
journal={IEEE Transactions on Information Theory}, 
title={Covert Communication Over Noisy Channels: A Resolvability Perspective}, 
year={2016},
volume={62},
number={5},
pages={2334-2354},
doi={10.1109/TIT.2016.2530089}}

@ARTICLE{ligong_first,  author={Wang, Ligong and Wornell, Gregory W. and Zheng, Lizhong},  journal={IEEE Transactions on Information Theory},   title={Fundamental Limits of Communication With Low Probability of Detection},   year={2016},  volume={62},  number={6},  pages={3493-3503},  doi={10.1109/TIT.2016.2548471}}

% Keyless

@INPROCEEDINGS{che_keyless,
  author={Che, Pak Hou and Bakshi, Mayank and Jaggi, Sidharth},
  booktitle={2013 IEEE International Symposium on Information Theory}, 
  title={Reliable deniable communication: Hiding messages in noise}, 
  year={2013},
  volume={},
  number={},
  pages={2945-2949},
  doi={10.1109/ISIT.2013.6620765}}

@INPROCEEDINGS{bloch_keyless,
  author={Arumugam, Keerthi Suria Kumar and Bloch, Matthieu R.},
  booktitle={2016 IEEE International Symposium on Information Theory (ISIT)}, 
  title={Keyless covert communication over Multiple-Access Channels}, 
  year={2016},
  volume={},
  number={},
  pages={2229-2233},
  doi={10.1109/ISIT.2016.7541695}}

@ARTICLE{bloch_asymp_keyless_to_del,
  author={Zivarifard, Hassan and Bloch, Matthieu R. and Nosratinia, Aria},
  journal={IEEE Transactions on Information Theory}, 
  title={Keyless Covert Communication via Channel State Information}, 
  year={2022},
  volume={68},
  number={8},
  pages={5440-5474},
  doi={10.1109/TIT.2021.3135291}}

@ARTICLE{bloch_keyless_csi_journal,
  author={Zivarifard, Hassan and Bloch, Matthieu R. and Nosratinia, Aria},
  journal={IEEE Transactions on Information Theory}, 
  title={Keyless Covert Communication via Channel State Information}, 
  year={2022},
  volume={68},
  number={8},
  pages={5440-5474},
  keywords={Transmitters;Receivers;Encoding;Decoding;Reliability;Codes;Monte Carlo methods;Covert communication;channel state information;secret key;privacy amplification},
  doi={10.1109/TIT.2021.3135291}}


% Broadcast

@ARTICLE{bloch_journal_embedding_broadcast,
  author={Kumar Arumugam, Keerthi Suria and Bloch, Matthieu R.},
  journal={IEEE Transactions on Information Forensics and Security}, 
  title={Embedding Covert Information in Broadcast Communications}, 
  year={2019},
  volume={14},
  number={10},
  pages={2787-2801},
  doi={10.1109/TIFS.2019.2907190}}
  
  @INPROCEEDINGS{ligong_broadcast,  author={Kibloff, David and Perlaza, Samir M. and Wang, Ligong},  booktitle={2019 IEEE International Symposium on Information Theory (ISIT)},   title={Embedding Covert Information on a Given Broadcast Code},   year={2019},  volume={},  number={},  pages={2169-2173},  doi={10.1109/ISIT.2019.8849435}}

% MAC

@ARTICLE{bloch_k_users_mac,
  author={Arumugam, Keerthi Suria Kumar and Bloch, Matthieu R.},
  journal={IEEE Transactions on Information Theory}, 
  title={Covert Communication Over a  $K$ -User Multiple-Access Channel}, 
  year={2019},
  volume={65},
  number={11},
  pages={7020-7044},
  doi={10.1109/TIT.2019.2930484}
  }

%%% MAC bloch conference.
    % @ARTICLE{bloch_k_users_mac,  
  % author={Arumugam, Keerthi Suria Kumar and Bloch, Matthieu R.},  
  % journal={IEEE Transactions on Information Theory},   
  % title={Covert Communication Over a  $K$ -User Multiple-Access Channel},   year={2019},  
  % volume={65},  
  % number={11},  
  % pages={7020-7044},  
  % doi={10.1109/TIT.2019.2930484}}

  @ARTICLE{sang_multiple_overt_superposition_covert_on_overt,
  author={Kim, Sang Wu and Ta, Hien Q.},
  journal={IEEE Transactions on Communications}, 
  title={Covert Communications Over Multiple Overt Channels}, 
  year={2022},
  volume={70},
  number={2},
  pages={1112-1124},
  doi={10.1109/TCOMM.2021.3127532}}

  @ARTICLE{sang_noma_multiple_overt_superposition_covert_on_overt,
  author={Ta, Hien Quang and Ho-Van, Khuong and Da Costa, Daniel Benevides and Kim, Sang Wu and Oh, Hoon},
  journal={IEEE Access}, 
  title={Covert Communications Over Non-Orthogonal Multiple Overt Channels}, 
  year={2022},
  volume={10},
  number={},
  pages={122361-122375},
  doi={10.1109/ACCESS.2022.3223357}}

@book{cover,
	author = {T.~M.~Cover and J.~A.~Thomas},
	title = {Elements of Information Theory, 2nd Ed},
	publisher={Wiley},
	place={New York, USA},
	year = {2006}
}

@book{Csiszarbook,
	author={I.~{Csisz\'ar} and J.~K\"orner},
	title={Information theory: coding theorems for discrete memoryless systems},
	publisher={Cambridge University Press},
	place={Cambridge},
	year={2011}
}

% Jammers
@ARTICLE{bash_uninformed_jammer,
  author={Sobers, Tamara V. and Bash, Boulat A. and Guha, Saikat and Towsley, Don and Goeckel, Dennis},
  journal={IEEE Transactions on Wireless Communications}, 
  title={Covert Communication in the Presence of an Uninformed Jammer}, 
  year={2017},
  volume={16},
  number={9},
  pages={6193-6206},
  doi={10.1109/TWC.2017.2720736}}

@INPROCEEDINGS{bash_uninformed_informed_coordinated_jammer,
  author={ZivariFard, Hassan and Bloch, Matthieu R. and Nosratinia, Aria},
  booktitle={2022 IEEE International Symposium on Information Theory (ISIT)}, 
  title={Covert Communication in the Presence of an Uninformed, Informed, and Coordinated Jammer}, 
  year={2022},
  volume={},
  number={},
  pages={306-311},
  keywords={Transmitters;Symbols;Receivers;Data communication;Jamming;Lifting equipment;Information theory},
  doi={10.1109/ISIT50566.2022.9834682}}
  
  @ARTICLE{shmuel_multi_antennas_jammer,
  author={Shmuel, Ori and Cohen, Asaf and Gurewitz, Omer},
  journal={IEEE Transactions on Communications}, 
  title={Multi-Antenna Jamming in Covert Communication}, 
  year={2021},
  volume={69},
  number={7},
  pages={4644-4658},
  doi={10.1109/TCOMM.2021.3067386}}

  % channel uncertainty
  @INPROCEEDINGS{che_uncertainty,
  author={Che, Pak Hou and Bakshi, Mayank and Chan, Chung and Jaggi, Sidharth},
  booktitle={2014 IEEE Information Theory Workshop (ITW 2014)}, 
  title={Reliable deniable communication with channel uncertainty}, 
  year={2014},
  volume={},
  number={},
  pages={30-34},
  doi={10.1109/ITW.2014.6970786}}

  % CSI
  
  @ARTICLE{ligong_csi_uncertainty_tx,
  author={Lee, Si-Hyeon and Wang, Ligong and Khisti, Ashish and Wornell, Gregory W.},
  journal={IEEE Transactions on Information Forensics and Security}, 
  title={Covert Communication With Channel-State Information at the Transmitter}, 
  year={2018},
  volume={13},
  number={9},
  pages={2310-2319},
  doi={10.1109/TIFS.2018.2818650}}

  
@INPROCEEDINGS{bloch_coop_jammer,
  author={ZivariFard, Hassan and Bloch, Matthieu R. and Nosratinia, Aria},
  booktitle={2021 IEEE International Symposium on Information Theory (ISIT)}, 
  title={Covert Communication via Non-Causal Cribbing from a Cooperative Jammer}, 
  year={2021},
  volume={},
  number={},
  pages={202-207},
  doi={10.1109/ISIT45174.2021.9517883}}



@INPROCEEDINGS{bloch_keyless_csi,
  author={ZivariFard, Hassan and Bloch, Matthieu and Nosratinia, Aria},
  booktitle={2019 IEEE Information Theory Workshop (ITW)}, 
  title={Keyless Covert Communication in the Presence of Non-causal Channel State Information}, 
  year={2019},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/ITW44776.2019.8989317}}


@article{bloch_keyless_csi_journal_arxiv,
  author    = {Hassan ZivariFard and
               Matthieu R. Bloch and
               Aria Nosratinia},
  title     = {Keyless Covert Communication via Channel State Information},
  journal   = {CoRR},
  volume    = {abs/2003.03308},
  year      = {2020},
  url       = {https://arxiv.org/abs/2003.03308},
  eprinttype = {arXiv},
  eprint    = {2003.03308},
  timestamp = {Tue, 10 Mar 2020 13:33:48 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2003-03308.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


  
% books and phd dissertations
@BOOK{livre_rioul,
  author = {Olivier Rioul},
  year = {2007},
  title = {Théorie de l'information et du codage},
  publisher = {Hermes Science  - Lavoisier}
}


@phdthesis{hou_phdthesis,
    title    = {Coding for relay networks and effective secrecy for wire-tap channels},
    school   = {Technischen Universitat München},
    author   = {J. Hou},
    year     = {2014},
    type     = {{PhD} dissertation},
}

% Quantum

@INPROCEEDINGS{bash_quantum,
  author={Sheikholeslami, Azadeh and Bash, Boulat A. and Towsley, Don and Goeckel, Dennis and Guha, Saikat},
  booktitle={2016 IEEE International Symposium on Information Theory (ISIT)}, 
  title={Covert communication over classical-quantum channels}, 
  year={2016},
  volume={},
  number={},
  pages={2064-2068},
  doi={10.1109/ISIT.2016.7541662}}

% others
@book{lehmann2005hypothesistesting,
  added-at = {2010-03-21T00:26:58.000+0100},
  address = {New York},
  author = {Lehmann, E. L. and Romano, Joseph P.},
  biburl = {https://www.bibsonomy.org/bibtex/28201f448d2af0d4fd287181787c0d128/peter.ralph},
  edition = {Third},
  interhash = {9517319578e44006dcf98ae19f983394},
  intrahash = {8201f448d2af0d4fd287181787c0d128},
  isbn = {0-387-98864-5},
  keywords = {book reference statistics},
  mrclass = {62-02 (62C05 62F03 62H15)},
  mrnumber = {MR2135927 (2006m:62005)},
  pages = {xiv+784},
  publisher = {Springer},
  series = {Springer Texts in Statistics},
  timestamp = {2010-03-21T00:26:59.000+0100},
  title = {Testing statistical hypotheses},
  year = 2005
}

@ARTICLE{tin_paper,
  author={Cho, Kang-Hee and Lee, Si-Hyeon},
  journal={IEEE Transactions on Information Forensics and Security}, 
  title={Treating Interference as Noise Is Optimal for Covert Communication Over Interference Channels}, 
  year={2021},
  volume={16},
  number={},
  pages={322-332},
  doi={10.1109/TIFS.2020.3013213}}

@article{ours_first_arxiv,
  title={Mixing a Covert and a Non-Covert User},
  author={Bounhar, Abdelaziz and Sarkiss, Mireille and Wigger, Mich{\`e}le},
  journal={arXiv preprint arXiv:2305.06268},
  year={2023}
}

@INPROCEEDINGS{ours_first,
  author={Bounhar, Abdelaziz and Sarkiss, Mireille and Wigger, Michèle},
  booktitle={2023 IEEE International Symposium on Information Theory (ISIT)}, 
  title={Mixing a Covert and a Non-Covert User}, 
  year={2023},
  volume={},
  number={},
  pages={2577-2582},
  keywords={Information theory},
  doi={10.1109/ISIT54713.2023.10206954}}

% for globecom

@ARTICLE{shannon_seperation,
  author={Shannon, C. E.},
  journal={The Bell System Technical Journal}, 
  title={A mathematical theory of communication}, 
  year={1948},
  volume={27},
  number={3},
  pages={379-423},
  keywords={},
  doi={10.1002/j.1538-7305.1948.tb01338.x}}

% finite blocklentgh
@ARTICLE{verdu_lossy_jscc_finite_blocklength,
  author={Kostina, Victoria and Verdú, Sergio},
  journal={IEEE Transactions on Information Theory}, 
  title={Lossy Joint Source-Channel Coding in the Finite Blocklength Regime}, 
  year={2013},
  volume={59},
  number={5},
  pages={2545-2575},
  keywords={Joints;Channel coding;Dispersion;Gaussian approximation;Source coding;Distortion measurement;Achievability;converse;finite blocklength regime;joint source-channel coding (JSCC);lossy source coding;memoryless sources;rate-distortion theory;Shannon theory},
  doi={10.1109/TIT.2013.2238657}}

% Gunduz
@ARTICLE{gunduz_beyond_transmitting_bits,
  author={Gündüz, Deniz and Qin, Zhijin and Aguerri, Inaki Estella and Dhillon, Harpreet S. and Yang, Zhaohui and Yener, Aylin and Wong, Kai Kit and Chae, Chan-Byoung},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Beyond Transmitting Bits: Context, Semantics, and Task-Oriented Communications}, 
  year={2023},
  volume={41},
  number={1},
  pages={5-41},
  keywords={Semantics;Task analysis;Syntactics;Receivers;Symbols;Reliability theory;Communication networks;6G;semantic communications;semantic distortion;goal-oriented communications;joint source-channel coding;deep learning (DL);rate-distortion theory;information bottleneck (IB);pragmatic communications;remote inference;distributed learning},
  doi={10.1109/JSAC.2022.3223408}}

@misc{deep_jscc_vit_image_gunduz,
      title={Deep Joint Source-Channel Coding for Adaptive Image Transmission over MIMO Channels}, 
      author={Haotian Wu and Yulin Shao and Chenghong Bian and Krystian Mikolajczyk and Deniz Gündüz},
      year={2024},
      eprint={2309.00470},
      archivePrefix={arXiv},
      primaryClass={cs.IT}
}

@INPROCEEDINGS{deep_secure_jscc_image_gunduz,
  author={Tung, Tze-Yang and Gündüz, Deniz},
  booktitle={ICC 2023 - IEEE International Conference on Communications}, 
  title={Deep Joint Source-Channel and Encryption Coding: Secure Semantic Communications}, 
  year={2023},
  volume={},
  number={},
  pages={5620-5625},
  keywords={Wireless communication;Image quality;Image coding;Image communication;Semantics;Distortion;Parity check codes},
  doi={10.1109/ICC45041.2023.10278612}}

@ARTICLE{deep_jscc_img_retrieval_at_edge_gunduz,
  author={Jankowski, Mikolaj and Gündüz, Deniz and Mikolajczyk, Krystian},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Wireless Image Retrieval at the Edge}, 
  year={2021},
  volume={39},
  number={1},
  pages={89-100},
  keywords={Image edge detection;Servers;Task analysis;Wireless communication;Performance evaluation;Image coding;Feature extraction;Deep learning;Internet of Things;image retrieval;joint source-channel coding;person re-identification},
  doi={10.1109/JSAC.2020.3036955}}

@ARTICLE{deep_jscc_img_generative_gunduz,
  author={Erdemir, Ecenaz and Tung, Tze-Yang and Dragotti, Pier Luigi and Gündüz, Deniz},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Generative Joint Source-Channel Coding for Semantic Image Transmission}, 
  year={2023},
  volume={41},
  number={8},
  pages={2645-2657},
  keywords={Wireless communication;Image reconstruction;Generators;Distortion;Training;Channel coding;Image coding;Semantic communication;wireless communication;joint source-channel coding;perceptual similarity;generative adversarial networks;inverse problems;StyleGAN},
  doi={10.1109/JSAC.2023.3288243}}

@INPROCEEDINGS{deep_wiretap_secure_jscc_gunduz,
  author={Erdemir, Ecenaz and Dragotti, Pier Luigi and Gündüz, Deniz},
  booktitle={ICASSP 2022 - 2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={Privacy-Aware Communication over a Wiretap Channel with Generative Networks}, 
  year={2022},
  volume={},
  number={},
  pages={2989-2993},
  keywords={Wireless communication;Wireless sensor networks;Simulation;Conferences;Receivers;Information processing;Signal processing;Privacy-utility trade-off;wiretap channel;physical layer security;generative networks;variational autoencoders},
  doi={10.1109/ICASSP43922.2022.9747068}}

@INPROCEEDINGS{deep_min_leakage_secure_jscc_gunduz,
  author={Marchioro, Thomas and Laurenti, Nicola and Gündüz, Deniz},
  booktitle={ICASSP 2020 - 2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={Adversarial Networks for Secure Wireless Communications}, 
  year={2020},
  volume={},
  number={},
  pages={8748-8752},
  keywords={Wireless communication;Neural networks;Receivers;Encoding;Security;Noise measurement;Speech processing;security;wiretap channel;convolutional neural networks;generative adversarial networks},
  doi={10.1109/ICASSP40776.2020.9053216}}





% others

@INPROCEEDINGS{deep_jscc_txt_1,
  author={Farsad, Nariman and Rao, Milind and Goldsmith, Andrea},
  booktitle={2018 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={Deep Learning for Joint Source-Channel Coding of Text}, 
  year={2018},
  volume={},
  number={},
  pages={2326-2330},
  keywords={Decoding;Channel coding;Machine learning;Source coding;Image coding;Training;deep learning;natural language processing;Joint source-channel coding},
  doi={10.1109/ICASSP.2018.8461983}}


@INPROCEEDINGS{9154322,
  author={Park, Sangwoo and Simeone, Osvaldo and Kang, Joonhyuk},
  booktitle={2020 IEEE 21st International Workshop on Signal Processing Advances in Wireless Communications (SPAWC)}, 
  title={End-to-End Fast Training of Communication Links Without a Channel Model via Online Meta-Learning}, 
  year={2020},
  volume={},
  number={},
  pages={1-5},
  keywords={Training;Decoding;Receivers;Transmitters;Testing;Channel models;Neural networks;Machine learning;autoencoder;fading channels;meta-learning},
  doi={10.1109/SPAWC48557.2020.9154322}}


@ARTICLE{deep_jscc_txt_2,
  author={Xie, Huiqiang and Qin, Zhijin and Li, Geoffrey Ye and Juang, Biing-Hwang},
  journal={IEEE Transactions on Signal Processing}, 
  title={Deep Learning Enabled Semantic Communication Systems}, 
  year={2021},
  volume={69},
  number={},
  pages={2663-2675},
  keywords={Semantics;Communication systems;Receivers;Transmitters;Task analysis;Encoding;Training;Deep learning;end-to-end communication;semantic communication;transfer learning;Transformer},
  doi={10.1109/TSP.2021.3071210}}

@ARTICLE{deep_jscc_video,
  author={Jiang, Peiwen and Wen, Chao-Kai and Jin, Shi and Li, Geoffrey Ye},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Wireless Semantic Communications for Video Conferencing}, 
  year={2023},
  volume={41},
  number={1},
  pages={230-244},
  keywords={Semantics;Symbols;Static VAr compensators;Wireless communication;Videoconferences;Detectors;Feature extraction;IR-HARQ;CSI feedback;semantic communication;video conferencing;facial keypoints},
  doi={10.1109/JSAC.2022.3221968}}


% adversarial robustness

@ARTICLE{phy_layer_adv_robustness_1,
  author={Nan, Guoshun and Li, Zhichun and Zhai, Jinli and Cui, Qimei and Chen, Gong and Du, Xin and Zhang, Xuefei and Tao, Xiaofeng and Han, Zhu and Quek, Tony Q. S.},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Physical-Layer Adversarial Robustness for Deep Learning-Based Semantic Communications}, 
  year={2023},
  volume={41},
  number={8},
  pages={2592-2608},
  keywords={Semantics;Communication systems;Wireless communication;Perturbation methods;Robustness;Communication system security;Receivers;Deep learning;semantic communications;physical-layer attacks;adversarial robustness;end-to-end communication systems},
  doi={10.1109/JSAC.2023.3288249}}

@article{semantic_adv,
  title={Boosting physical layer black-box attacks with semantic adversaries in semantic communications},
  author={Li, Zeju and Liu, Xinghan and Nan, Guoshun and Zhou, Jinfei and Lyu, Xinchen and Cui, Qimei and Tao, Xiaofeng},
  journal={arXiv preprint arXiv:2303.16523},
  year={2023}
}

% attacks on DNN

@article{attack_dnn_1,
  title={Intriguing properties of neural networks},
  author={Szegedy, Christian and Zaremba, Wojciech and Sutskever, Ilya and Bruna, Joan and Erhan, Dumitru and Goodfellow, Ian and Fergus, Rob},
  journal={arXiv preprint arXiv:1312.6199},
  year={2013}
}

@ARTICLE{mnist_paper,
  author={Lecun, Y. and Bottou, L. and Bengio, Y. and Haffner, P.},
  journal={Proceedings of the IEEE}, 
  title={Gradient-based learning applied to document recognition}, 
  year={1998},
  volume={86},
  number={11},
  pages={2278-2324},
  keywords={Neural networks;Pattern recognition;Machine learning;Optical character recognition software;Character recognition;Feature extraction;Multi-layer neural network;Optical computing;Hidden Markov models;Principal component analysis},
  doi={10.1109/5.726791}}

@article{adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@book{book_Testing_Statistical_Hypotheses,
  title={Testing Statistical Hypotheses},
  author={Lehmann, E. L. and Romano, J. P.},
  year={2005},
  publisher={Springer-Verlag},
  address={New York, NY, USA}
}


@article{soft_histogram,
  title={Quantum-chemical insights from deep tensor neural networks},
  author={Sch{\"u}tt, Kristof T and Arbabzadah, Farhad and Chmiela, Stefan and M{\"u}ller, Klaus R and Tkatchenko, Alexandre},
  journal={Nature communications},
  volume={8},
  number={1},
  pages={13890},
  year={2017},
  publisher={Nature Publishing Group UK London}
}

@article{ste_paper,
  author       = {Yoshua Bengio and
                  Nicholas L{\'{e}}onard and
                  Aaron C. Courville},
  title        = {Estimating or Propagating Gradients Through Stochastic Neurons for
                  Conditional Computation},
  journal      = {CoRR},
  volume       = {abs/1308.3432},
  year         = {2013},
  url          = {http://arxiv.org/abs/1308.3432},
  eprinttype    = {arXiv},
  eprint       = {1308.3432},
  timestamp    = {Mon, 13 Aug 2018 16:47:35 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/BengioLC13.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

 @ARTICLE{song_cuff_likelihood_encoder,
  author={Song, Eva C. and Cuff, Paul and Poor, H. Vincent},
  journal={IEEE Transactions on Information Theory}, 
  title={The Likelihood Encoder for Lossy Compression}, 
  year={2016},
  volume={62},
  number={4},
  pages={1836-1849},
  keywords={Distortion;Rate-distortion;Decoding;Source coding;Context;Indexes;Markov processes;Berger-Tung;likelihood encoder;rate-distortion theory;soft-covering;source coding;Wyner-Ziv;Berger-Tung;likelihood encoder;rate-distortion theory;soft-covering;source coding;Wyner-Ziv},
  doi={10.1109/TIT.2016.2529657}}
